Benefits of Stabilization versus Rollback in Eventually Consistent Key-Value Stores

In this paper, we evaluate and compare the performance of two approaches, namely self-stabilization and rollback, to handling consistency violation faults (cvf) that occurred when a distributed program is executed on eventually consistent key-value store. We observe that self-stabilization is usually better than rollbacks in our experiments. Moreover, when we aggressively allow more cvf in exchange of eliminating mechanisms for guaranteeing atomicity requirements of actions, we observe the programs in our case studies achieve a speedup between 2--15 times compared with the standard implementation. We also analyze different factors that contribute to the results. Our results and analysis are useful in helping a system designer choose proper design options for their program.

==> experiment-analysis.tex <==
\begin{itemize}
    \item In the later round of stabilization algorithm, only a small number of nodes need to change their states and most other nodes are unchanged (stable nodes).
    By not using mechanism for exclusive access, the clients scan over these stable nodes quickly (since obtaining exclusive access is usually the most time consuming operation for each node). Therefore, the computation is speedup.
    \item Also some \cvf are not harmful. As an example, consider a scenario in graph coloring problem where client $C1$ reads the state/color of node $j$ while client $C2$ is updating the state/color of $j$. This is a \cvf since in sequential consistency, this should not happen when the clients employ exclusive access mechanisms. However, $C2$ does not change the state/color of $j$ since its color is different from all the neighbors. So the state value $j$ read by $C1$ is still consistent.
    For another example, consider a \cvf corresponding to the reading of an inconsistent value of some variables that results in guard $g$ of an action $g \longrightarrow st$ to evaluate to false. The effect of such \cvf is the stuttering of the same state. In stabilization approach, the computation of the program is unaffected by such harmless \cvf while in the detect-rollback approach, since the monitors are not able to classify harmful and harmless \cvf, they triggers unnecessary rollbacks. 
    \item Another factor is the monitors in detect-rollback approach suffers from false positives in detection of \cvf. Therefore, the detect-rollback approach may be not efficient as the stabilization approach.
    \item The detect-rollback approach also is limited to detection of linear and semi-linear predicates.
    \item The benefit of rollback in the random partition depends on specific partition.
    \item Eventual with aggressive stabilization provides the best performance. However, it increases the chance of \cvf and create some \cvf's that are difficult to recover.
    
\end{itemize}


% \textbf{Nature of problems}
% problem where a change has cascading effect like maximal matching

% Problem where a change is local like coloring

% \textbf{Nature of input graph}
% Highly connected graphs such social graph

% Less connected graphs such as planar graph, regular graphs

% \textbf{Impact of graph partition schemes}
% Using Metis partition: requires pre-processing.

% Using normal partition

% The difference between R1W3-ME and R1W1-ME reflects the difference between sequential consistency and eventual consistency. The difference between R1W1-ME and R1W1-noME shows the amount of time needed for coordination between the clients. This amount of time constitute the majority of the computation time. And therefore, the read phase constitute the majority of time of a task.



==> related-work.tex <==
Compare to \cite{NCKD2018LADC} and \cite{NKD2019ICDCN}, this work examine the two approaches with more problems and test cases.

\todo{Skip this if space is tight}
